MetaSketch: Wireless Semantic Segmentation by Metamaterial Surfaces

Semantic segmentation is a process of partitioning an image into multiple segments for recognizing humans and objects, which can be widely applied in scenarios such as healthcare and safety monitoring. To avoid privacy violation, using RF signals instead of an image for human and object recognition has gained increasing attention. However, human and object recognition by using RF signals is usually a passive signal collection and analysis process without changing the radio environment, and the recognition accuracy is restricted significantly by unwanted multi-path fading, and/or the limited number of independent channels between RF transceivers in uncontrollable radio environments. This paper introduces MetaSketch, a novel RF-sensing system that performs semantic recognition and segmentation for humans and objects by making the radio environment reconfigurable. A metamaterial surface is incorporated into MetaSketch and diversifies the information carried by RF signals. Using compressive sensing techniques, MetaSketch reconstructs a point cloud consisting of the reflection coefficients of humans and objects at different spatial points, and recognizes the semantic meaning of the points by using symmetric multilayer perceptron groups. Our evaluation results show that MetaSketch is capable of generating favorable radio environments and extracting exact point clouds, and labeling the semantic meaning of the points with an average error rate of less than 1% in an indoor space.

==> ms <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{shapiro1992computer}
L.~Shapiro, \emph{Computer vision and image processing}.\hskip 1em plus 0.5em
  minus 0.4em\relax San Diego, CA: Academic Press, 1992.

\bibitem{zhang2019Feasibility}
D.~Zhang, J.~Wang, J.~Jang, J.~Zhang, and S.~Kumar, ``On the feasibility of
  {Wi-Fi} based material sensing,'' in \emph{Proceedings of the 25th Annual
  International Conference on Mobile Computing and Networking~(MobiCom'18)},
  Los Cabos, Mexico, Oct. 2019.

\bibitem{jiang2018towards}
W.~Jiang, C.~Miao, F.~Ma, S.~Yao, Y.~Wang, Y.~Yuan, H.~Xue, C.~Song, X.~Ma,
  D.~Koutsonikolas, and et~al., ``Towards environment independent device free
  human activity recognition,'' in \emph{Proceedings of the 24th Annual
  International Conference on Mobile Computing and Networking~(MobiCom'18)},
  New Delhi, India, Oct. 2018.

\bibitem{Zhang2018CrossSense}
J.~Zhang, Z.~Tang, M.~Li, D.~Fang, P.~Nurmi, and Z.~Wang, ``Crosssense: Towards
  cross-site and large-scale {WiFi} sensing,'' in \emph{Proceedings of the 24th
  Annual International Conference on Mobile Computing and
  Networking~(MobiCom'18)}, New Delhi, India, Oct. 2018.

\bibitem{Hsu2019Enabling}
C.-Y. Hsu, R.~Hristov, G.-H. Lee, M.~Zhao, and D.~Katabi, ``Enabling
  identification and behavioral sensing in homes using radio reflections,'' in
  \emph{Proceedings of the 2019 CHI Conference on Human Factors in Computing
  Systems~(CHI'19)}, Glasgow, Scotland UK, May 2019.

\bibitem{zhao2018through}
M.~Zhao, T.~Li, M.~Abu~Alsheikh, Y.~Tian, H.~Zhao, A.~Torralba, and D.~Katabi,
  ``Through-wall human pose estimation using radio signals,'' in
  \emph{Proceedings of the IEEE Conference on Computer Vision and Pattern
  Recognition~(CVPR'18)}, Salt Lake City, Utah, Jun. 2018.

\bibitem{adib2015capturing}
F.~Adib, C.-Y. Hsu, H.~Mao, D.~Katabi, and F.~Durand, ``Capturing the human
  figure through a wall,'' \emph{ACM Transactions on Graphics}, vol.~34, no.~6,
  p. 219, Oct. 2015.

\bibitem{zhao2018rf}
M.~Zhao, Y.~Tian, H.~Zhao, M.~A. Alsheikh, T.~Li, R.~Hristov, Z.~Kabelac,
  D.~Katabi, and A.~Torralba, ``Rf-based 3d skeletons,'' in \emph{Proceedings
  of the 2018 Conference of the ACM Special Interest Group~(SIGCOMM'18)}, New
  York, New York, USA, Aug. 2018.

\bibitem{PedrossEngel2018Orthogonal}
A.~Pedross-Engel, D.~Arnitz, J.~N. Gollub, O.~Yurduseven, K.~P. Trofatter,
  M.~F. Imani, T.~Sleasman, M.~Boyarsky, X.~Fu, D.~L. Marks, D.~R. Smith, and
  M.~S. Reynolds, ``Orthogonal coded active illumination for millimeter wave,
  massive-{MIMO} computational imaging with metasurface antennas,'' \emph{IEEE
  Transactions on Computational Imaging}, vol.~4, no.~2, pp. 184--193, Jun.
  2018.

\bibitem{honma2018Human}
N.~{Honma}, D.~{Sasakawa}, N.~{Shiraki}, T.~{Nakayama}, and S.~{Iizuka},
  ``Human monitoring using {MIMO} radar,'' in \emph{Proceedings of the 2018
  IEEE International Workshop on Electromagnetics: Applications and Student
  Innovation Competition~(iWEM'18)}, Nagoya, Japan, Aug. 2018.

\bibitem{li2020programmable}
Z.~Li, Y.~Xie, L.~Shangguan, R.~I. Zelaya, J.~Gummeson, W.~Hu, and K.~Jamieson,
  ``Programmable radio environments with large arrays of inexpensive
  antennas,'' \emph{GetMobile: Mobile Computing and Communications}, vol.~23,
  no.~3, pp. 23--27, Sep. 2019.

\bibitem{Renzo2019Smart}
M.~Di~Renzo, M.~Debbah, D.-T. Phan-Huy, A.~Zappone, M.-S. Alouini, C.~Yuen,
  V.~Sciancalepore, G.~C. Alexandropoulos, J.~Hoydis, H.~Gacanin, J.~D. Rosny,
  A.~Bounceu, G.~Lerosey, and M.~Fink, ``Smart radio environments empowered by
  ai reconfigurable meta-surfaces: An idea whose time has come,''
  \emph{arXiv:1903.08925}.

\bibitem{adib2015multi}
F.~Adib, Z.~Kabelac, and D.~Katabi, ``Multi-person localization via {RF} body
  reflections,'' in \emph{Proceedings of the 12th {USENIX} Symposium on
  Networked Systems Design and Implementation~(NSDI'15)}, Oakland, CA, May
  2015.

\bibitem{patwari2010rf}
N.~Patwari and J.~Wilson, ``{RF} sensor networks for device-free localization:
  Measurements, models, and algorithms,'' \emph{Proceedings of the IEEE},
  vol.~98, no.~11, pp. 1961--1973, Nov. 2010.

\bibitem{Kellogg2014Bringing}
B.~Kellogg, V.~Talla, and S.~Gollakota, ``Bringing gesture recognition to all
  devices,'' in \emph{Proceedings of the 11th {USENIX} Symposium on Networked
  Systems Design and Implementation~(NSDI'14)}, Seattle, WA, Apr. 2014.

\bibitem{sigg2013rf}
S.~Sigg, M.~Scholz, S.~Shi, Y.~Ji, and M.~Beigl, ``Rf-sensing of activities
  from non-cooperative subjects in device-free recognition systems using
  ambient and local signals,'' \emph{IEEE Transactions on Mobile Computing},
  vol.~13, no.~4, pp. 907--920, Feb. 2013.

\bibitem{lien2016soli}
J.~Lien, N.~Gillian, M.~E. Karagozler, P.~Amihood, C.~Schwesig, E.~Olson,
  H.~Raja, and I.~Poupyrev, ``Soli: Ubiquitous gesture sensing with millimeter
  wave radar,'' \emph{ACM Transactions on Graphics}, vol.~35, no.~4, p. 142,
  Jul. 2016.

\bibitem{Wang2016RF-Fall}
H.~Wang, D.~Zhang, Y.~Wang, J.~Ma, Y.~Wang, and S.~Li, ``{RT-Fall}: A real-time
  and contactless fall detection system with commodity {WiFi} devices,''
  \emph{IEEE Transaction Mobile Computing}, vol.~16, no.~2, pp. 511--526, Dec.
  2016.

\bibitem{tian2018rf}
Y.~Tian, G.-H. Lee, H.~He, C.-Y. Hsu, and D.~Katabi, ``{RF-based} fall
  monitoring using convolutional neural networks,'' \emph{Proceedings of the
  ACM on Interactive, Mobile, Wearable and Ubiquitous Technologies}, vol.~2,
  no.~3, pp. 1--24, Sep. 2018.

\bibitem{Gollub2017Large}
J.~N. Gollub, O.~Yurduseven, K.~P. Trofatter, D.~Arnitz, M.~F. Imani,
  T.~Sleasman, M.~Boyarsky, A.~Rose, A.~Pedross-Engel, H.~Odabasi,
  T.~Zvolensky, G.~Lipworth, D.~Brady, D.~L. Marks, M.~S. Reynolds, and D.~R.
  Smith, ``Large metasurface aperture for millimeter wave computational imaging
  at the human-scale,'' \emph{Scientific Reports}, vol.~7, no.~1, p. 42650,
  Feb.

\bibitem{Long_2015_CVPR}
J.~Long, E.~Shelhamer, and T.~Darrell, ``Fully convolutional networks for
  semantic segmentation,'' in \emph{Proceedings of the IEEE Conference on
  Computer Vision and Pattern Recognition~(CVPR'15)}, Boston, MA, Jun. 2015.

\bibitem{ren2015faster}
S.~Ren, K.~He, R.~Girshick, and J.~Sun, ``Faster {R-CNN}: Towards real-time
  object detection with region proposal networks,'' in \emph{Advances in Neural
  Information Processing Systems~(NIPS'15)}, Montreal, Canada, Dec. 2015.

\bibitem{Badrinarayanan2017SegNet}
V.~{Badrinarayanan}, A.~{Kendall}, and R.~{Cipolla}, ``{SegNet}: A deep
  convolutional encoder-decoder architecture for image segmentation,''
  \emph{IEEE Transactions on Pattern Analysis and Machine Intelligence},
  vol.~39, no.~12, pp. 2481--2495, Dec. 2017.

\bibitem{mehta2017vnect}
D.~Mehta, S.~Sridhar, O.~Sotnychenko, H.~Rhodin, M.~Shafiei, H.-P. Seidel,
  W.~Xu, D.~Casas, and C.~Theobalt, ``Vnect: Real-time {3D} human pose
  estimation with a single {RGB} camera,'' \emph{ACM Transactions on Graphics},
  vol.~36, no.~4, p.~44, Jul. 2017.

\bibitem{qi2017pointnet}
C.~R. Qi, H.~Su, K.~Mo, and L.~J. Guibas, ``Pointnet: Deep learning on point
  sets for 3d classification and segmentation,'' in \emph{Proceedings of the
  IEEE Conference on Computer Vision and Pattern Recognition~(CVPR'17)},
  Honolulu, Hawaii, Jul. 2017.

\bibitem{Zhou2017Short}
T.~Zhou, H.~Li, D.~Ye, J.~Huangfu, S.~Qiao, Y.~Sun, W.~Zhu, C.~Li, and L.~Ran,
  ``Short-range wireless localization based on meta-aperture assisted
  compressed sensing,'' \emph{IEEE Transactions on Microwave Theory and
  Technology}, vol.~65, no.~7, pp. 2516--2524, Jan. 2017.

\bibitem{cui2010metamaterials}
T.~J. Cui, D.~R. Smith, and R.~Liu, \emph{Metamaterials}.\hskip 1em plus 0.5em
  minus 0.4em\relax Boston, MA: Springer, 2010.

\bibitem{di2019hybrid}
B.~Di, H.~Zhang, L.~Song, Y.~Li, Z.~Han, and H.~V. Poor, ``Hybrid beamforming
  for reconfigurable intelligent surface based multi-user communications:
  Achievable rates with limited discrete phase shifts,''
  \emph{arXiv:1910.14328}.

\bibitem{tang2019wireless}
W.~Tang, M.~Z. Chen, X.~Chen, J.~Y. Dai, Y.~Han, M.~Di~Renzo, Y.~Zeng, S.~Jin,
  Q.~Cheng, and T.~J. Cui, ``Wireless communications with reconfigurable
  intelligent surface: Path loss modeling and experimental measurement,''
  \emph{arXiv:1911.05326}.

\bibitem{han_COMPRESSIVE}
Z.~Han, H.~Li, and W.~Yin, \emph{Compressive sensing for wireless
  networks}.\hskip 1em plus 0.5em minus 0.4em\relax New York, NY: Cambridge
  University Press, 2013.

\bibitem{candes2006stable}
E.~J. Candes, J.~K. Romberg, and T.~Tao, ``Stable signal recovery from
  incomplete and inaccurate measurements,'' \emph{Communications on Pure and
  Applied Mathematics}, vol.~59, no.~8, pp. 1207--1223, Mar. 2006.

\bibitem{Li2019Machine}
L.~Li, H.~Ruan, C.~Liu, Y.~Li, Y.~Shuang, A.~Al{\`u}, C.-W. Qiu, and T.~J. Cui,
  ``Machine-learning reprogrammable metasurface imager,'' \emph{Nature
  Communications}, vol.~10, no. 1082, pp. 1--8, Jun. 2019.

\bibitem{dai2015boxsup}
J.~Dai, K.~He, and J.~Sun, ``Boxsup: Exploiting bounding boxes to supervise
  convolutional networks for semantic segmentation,'' in \emph{Proceedings of
  the IEEE Conference on Computer Vision and Pattern Recognition~(CVPR'15)},
  Boston, MA, Jun. 2015.

\bibitem{goodfellow2016deep}
I.~Goodfellow, Y.~Bengio, and A.~Courvile, \emph{Deep learning}.\hskip 1em plus
  0.5em minus 0.4em\relax MIT Press: Cambridge, MA, 2016.

\bibitem{elad2007optimized}
M.~Elad, ``Optimized projections for compressed sensing,'' \emph{IEEE
  Transactions on Signal Processing}, vol.~55, no.~12, pp. 5695--5702, Nov.
  2007.

\bibitem{lewis2007implementing}
R.~M. Lewis, A.~Shepherd, and V.~Torczon, ``Implementing generating set search
  methods for linearly constrained minimization,'' \emph{SIAM Journal on
  Scientific Computing}, vol.~29, no.~6, pp. 2507--2530, Oct. 2007.

\bibitem{goldberg2006genetic}
D.~E. Goldberg, \emph{Genetic algorithms}.\hskip 1em plus 0.5em minus
  0.4em\relax Pearson Education India, 2006.

\bibitem{Boyd_CONVEX}
S.~Boyd and L.~Vandenberghe, \emph{Convex optimization}.\hskip 1em plus 0.5em
  minus 0.4em\relax Cambridge University Press: Cambridge, U.K., 2004.

\bibitem{Hirtenfelder2007Effective}
F.~{Hirtenfelder}, ``Effective antenna simulations using {CST MICROWAVE
  STUDIO$^\circledR$},'' in \emph{Proceedings of the 2nd International ITG
  Conference on Antennas~(INICA'07)}, Munich, Germany, Mar. 2007.

\bibitem{blossom2004gnu}
E.~Blossom, ``Gnu radio: Tools for exploring the radio frequency spectrum,''
  \emph{Linux Journal}, vol. 2004, no. 122, p.~4, Jun. 2004.

\bibitem{goldsmith2005wireless}
A.~Goldsmith, \emph{Wireless communications}.\hskip 1em plus 0.5em minus
  0.4em\relax Cambridge University Press, 2005.

\end{thebibliography}


==> sections/discussion.tex <==
\endinput
